Clova Baseline System for the VoxCeleb Speaker Recognition Challenge 2020

This report describes our submission to the VoxCeleb Speaker Recognition Challenge (VoxSRC) at Interspeech 2020. We perform a careful analysis of speaker recognition models based on the popular ResNet architecture, and train a number of variants using a range of loss functions. Our results show significant improvements over most existing works without the use of model ensemble or post-processing. We release the training code and pre-trained models as unofficial baselines for this year's challenge.

==> input_representation.tex <==
\begin{table}[h]
 \renewcommand\thetable{1}
 \caption{Hyper-parameters for input representation.}
  \centering
  \label{table:input}
  \begin{tabular}{r l }
  
  %\Xhline{2\arrayrulewidth}
  \toprule

   Hyper-parameter &  \\
  \hline
  frame length & 25ms\\
  
  shift size & 10ms \\
  
  number of FFT bins & 512\\
  
  number of filters & 64\\
  
  pre-emphasis & with 0.97 coefficient \\
  
  normalization & mean \& variance normalization\\
   \bottomrule
  \end{tabular}
\end{table}
